A novel approach to fluid-structure interaction simulations involving large translation and contact

In this work, we present a novel method for the mesh update in flow problems with moving boundaries, the phantom domain deformation mesh update method (PD-DMUM). The PD-DMUM is designed to avoid remeshing; even in the event of large, unidirectional displacements of boundaries. The method combines the concept of two mesh adaptation approaches: (1) The virtual ring shear-slip mesh updatemethod (VR-SSMUM); and (2) the elastic mesh update method (EMUM). As in the VR-SSMUM, the PD-DMUMextends the fluid domain by a phantom domain; the PD-DMUM can thus locally adapt the element density. Combined with the EMUM, the PD-DMUMallows the consideration of arbitrary boundary movements. In this work, we apply the PD-DMUM in two test cases. Within the first test case, we validate the PD-DMUM in a 2D Poiseuille flow on a moving background mesh. Subsequently the fluid-structure interaction (FSI) problem in the second test case serves as a proof of concept. More, we stress the advantages of the novel method with regard to conventional mesh update approaches.

==> sections/referenc.tex <==
\begin{thebibliography}{99.}

	\bibitem{Alauzet2013} F. Alauzet: Efficient moving mesh technique using generalized swapping. Proceedings of the 21st International Meshing Roundtable. Springer, Berlin, Heidelberg, 17--37 (2003).

	\bibitem{ElgetiSauerland2016}S. Elgeti, and H. Sauerland: Deforming fluid domains within the finite element method: five mesh-based tracking methods in comparison. Archives of Computational Methods in Engineering,  vol.  \textbf{23}, 323--361, (2016).

	\bibitem{FelippaParkFarhat1998} C.A. Felippa, K.C. Park, and C. Farhat: Partitioned analysis of coupled mechanical systems. Computer methods in applied mechanics and engineering, vol.  \textbf{190}, 3247--3270 (2001).

	\bibitem{HirtNichols1981} C.W. Hirt, and B.D. Nichols: Volume of fluid (VOF) method for the dynamics of free boundaries. Journal of computational physics, vol.  \textbf{39} 201--225 (1981).

	\bibitem{HostersEtAl2017}N. Hosters, J. Helmig, A. Stavrev, M. Behr, and S. Elgeti: Fluid-Structure Interaction with NURBS-Based Coupling. Computer Methods in Applied Mechanics and Engineering, vol.  \textbf{332} 520-539 (2018).

	\bibitem{HughesCottrellBazilevs2004} T.J.R. Hughes, J.A. Cottrell, and Y. Bazileves.  Isogeometric analysis: CAD, finite elements, NURBS, exact geometry and mesh refinement. Computer Methods in Applied Mechanics and Engineering, vol.  \textbf{194}, 4135--4195 (2005).

	\bibitem{HughesFrancaHulbert1989} T.J.R. Hughes, L.P. Franca, and G.M. Hulbert: A new finite element formulation for computational fluid dynamics: VIII. The Galerkin/least-squares method for advective-diffusive equations. Computer Methods in Applied Mechanics and Engineering, vol.  \textbf{73}, 173--189 (1989).

	\bibitem{JohnsonTezduyar1994} A.A. Johnson, and T.E. Tezduyar: Mesh update strategies in parallel finite element computations of flow problems with moving boundaries and interfaces. Computational Methods in Applied Mechanical Engineering, vol.  \textbf{119} 73--94 (1994).

	\bibitem{KeyPauliElgeti2018} F. Key, L. Pauli, and S. Elgeti: The Virtual Ring Shear-Slip Mesh Update Method. Computer and Fluids, vol.  \textbf{172}, 352--361 (2018).

	\bibitem{OsherSethian1988} S. Osher, and J.A. Sethian: Fronts propagating with curvature-dependent speed: algorithms based on Hamilton-Jacobi formulations. Journal of computational physics, vol.  \textbf{79} 12--49  (1988).

	\bibitem{PauliBehr2017} L. Pauli, and M. Behr: On stabilized space-time FEM for anisotropic meshes: Incompressible Navier--Stokes equations and applications to blood flow in medical devices. International Journal for Numerical Methods in Fluids, vol.  \textbf{85}, 189--209 (2017).

	\bibitem{PieglTiller1997} L. Piegl, and W. Tiller: The NURBS book. Springer, Berlin, (1997).

	\bibitem{TemizerWriggersHughes2011} I. Temizer, P. Wriggers, and T.J.R. Hughes: Contact Treatment in Isogeometric Analysis with NURBS". Computer Methods in Applied Mechanics and Engineering vol.  \textbf{200}, 1100--1112 (2011).

	\bibitem{TezduyarBehrLiou1992} T.E. Tezduyar, M. Behr, and J. Liou: A new strategy for finite element computations involving moving boundaries and interaces -- the deforming-spatial-domain/space-time procedure: I The concept and the preliminary numerical tests. Computational Methods in Applied Mechanical Engineering, vol.  \textbf{94}, 339--351 (1992).

	\bibitem{TezduyarEtAl1992}  T.E. Tezduyar, M. Behr, S. Mittal, and J. Liou: A new strategy for finite element computations involving moving boundaries and interaces -- the deforming-spatial-domain/space-time procedure: II Computations of free-surface flows, two-liquid flows, and flows with drifting cylinders. Computational Methods in Applied Mechanical Engineering, vol.  \textbf{94}, 353--371 (1992).

	\bibitem{Wall1999}W.A. Wall: Fluid-Struktur-Interaktionen mit stabilisierten Finiten Elementen". Institut f\"ur Baustatistik der Universit\"at Stuttgart, (1999).

	\bibitem{WangPersson2015} L. Wang, and PO. Persson: A high-order discontinuous Galerkin method with unstructured space-time meshes for two-dimensional compressible flows on domains with large deformations. Computers {\&} Fluids, vol. \text{118}, 53--68 (2015).

\end{thebibliography}

